Fray: An Efficient General-Purpose Concurrency Testing Platform for the JVM (Extended Version)

Concurrency bugs are hard to discover and reproduce. Prior work has developed sophisticated algorithms to search for concurrency bugs, such as partial order sampling (POS); however, fundamental limitations with existing platforms for concurrency control hinder effective testing of real-world software. We observe that the design space for concurrency control on managed code involves complex trade-offs between expressibility, applicability, and maintainability on the one hand, and bug-finding efficiency on the other hand. This paper presents Fray, a platform for performing push-button concurrency testing of data-race-free JVM programs. The key insight behind Fray is that effective controlled concurrency testing requires orchestrating thread interleavings without replacing existing concurrency primitives, while encoding their semantics for faithfully expressing the set of all possible program behaviors. Fray incorporates a novel concurrency control mechanism called shadow locking, designed to make controlled concurrency testing practical and efficient for JVM programs. In an empirical evaluation on 53 benchmark programs with known bugs (SCTBench and JaConTeBe), Fray with random search finds 70% more bugs than JPF and 77% more bugs than RR's chaos mode. We also demonstrate Fray's push-button applicability on 2,655 tests from Apache Kafka, Lucene, and Google Guava. In these mature projects, Fray successfully discovered 18 real-world concurrency bugs that can cause 363 tests to fail reproducibly.

==> relatedwork.tex <==
\section{Other Related Work}

\myparagraph{Concurrency Testing for Other Languages}
Coyote~\cite{Deligiannis23-coyote} is a concurrency testing framework for C\# programs using the Task Asynchronous Programming (TAP) model. It uses source or binary rewriting to replace concurrency primitives with custom implementations, similar to Lincheck. Likely due to similar complexities related to interoperability between applications and the runtime, Coyote does not control concurrency for C\# programs that use bare threads instead of the TAP model. For Rust programs, Shuttle~\cite{shuttle} and Loom~\cite{loom} enable concurrency testing using a similar design as Coyote; consequently, they share similar limits to push-button applicability. %See Section~\ref{sec:discussion-applicability} for an in-depth discussion about why this design is fundamentally hard to scale.


\myparagraph{Deterministic Record and Replay}
LEAP~\cite{Huang10-leap}, ORDER~\cite{Yang11-order}, and CARE~\cite{Jiang14-care} enable record-replay-debugging of concurrent Java executions via object-centric logging. However, they cannot be used to pick specific thread schedules for concurrency testing.

Kendo~\cite{Olszewski09-kendo}, CoreDet~\cite{Bergan10-coredet}, and DThreads~\cite{Liu11-dthreads} provide deterministic multithreading capabilities for C/C++ programs, but they cannot choose specific thread schedules and also cannot distinguish application threads from the managed runtime. 

\myparagraph{Flaky test detection}  Researchers have extensively studied the problem of \emph{flaky tests}~\cite{Bell18-deflaker, Lam19-idflakies, Parry21-flaky} that pass or fail non-deterministically. Shaker~\cite{Silva20-shaker} specifically targets flaky test detection due to concurrency issues, but it does not have any mechanism for controlling the non-determinism either for a systematic search or for deterministic replay.

%\myparagraph{Data-Race Detection} Researchers have developed many techniques to dynamically detect data races~\cite{Engler03-racerx, Flanagan09, Ocallahan03-hybrid, Kini17, Serebryany09-threadsanitizer}. RaceFuzzer~\cite{Sen08-racefuzzer} uses random testing to uncover data races in Java programs and replay the witness; however, it expects as input a set of racing pairs identified by imprecise static race detection tools. Further, it instruments almost every program instruction since it considers all possible interleavings including at memory accesses. 




\myparagraph{Scheduling algorithms for concurrency testing} Once controlled concurrency is feasible, popular search algorithms for bug finding include iterative context bounding~\cite{Musuvathi08-chess}, probabilistic concurrency testing (PCT)~\cite{Burckhardt10-pct}, partial-order sampling (POS)~\cite{Yuan18-pos}, coverage-driven testing (Maple)~\cite{Yu12-maple}. Our proposed framework can support any such strategy (ref.~\ref{sec:scheduling-search}).

Razzer~\cite{Jeong19-razzer}, DDRace~\cite{Yuan23-ddrace}, Conzzer~\cite{Jiang22-conzzer}, MUZZ~\cite{Chen20-muzz}, and RFF~\cite{Wolff24-rff} use various forms of fuzzing to find data races, deadlocks, or concurrency-related program crashes in C/C++ programs or the Linux kernel. 
% While these techniques focus on problems and assumptions inherent in C++/Linux environments, they do not directly apply to Java testing. 
% In principle, our proposed platform can be adapted for fuzz testing, though we have not implemented such methods. \rp{We can remove this line}
Periodical scheduling~\cite{Wen22-period} is a new concurrency testing technique that parallelizes threads in defined periods instead of searching over fixed sequences of interleavings. This is achieved through Linux’s deadline CPU scheduler, which is a system-level control.

% forgoes deterministic interleavings of thread sequences to parallelize selected threads in defined periods. This can be achieved via Linux’s deadline task scheduling, which is a system-level control. 


% can be used for fuzz testing as well, though we have not yet implemented any such technique.

%Although in principle our proposed platform can be used for fuzz testing as well, the prior work usually focuses on domains with different problems and assumptions.
